DecoPrompt : Decoding Prompts Reduces Hallucinations when Large Language Models Meet False Premises

While large language models (LLMs) have demonstrated increasing power, they have also called upon studies on their hallucinated outputs that deviate from factually correct statements. In this paper, we focus on one important scenario of false premises, where LLMs are distracted by misaligned claims although the model possesses the required factual knowledge to answer original questions accurately. Inspired by the observation that entropy of the false-premise prompt is closely related to its likelihood to elicit hallucination generation, we propose a new prompting algorithm, named DecoPrompt, to mitigate hallucination. DecoPrompt leverages LLMs to "decode" the false-premise prompts without really eliciting hallucination output from LLMs. We perform experiments on two datasets, demonstrating that DecoPrompt can reduce hallucinations effectively on outputs from different LLMs. Moreover, DecoPrompt exhibits cross-model transferability, which facilitates its applications to scenarios such as LLMs of large sizes or unavailable model logits.

==> latex/4_5_discussions.tex <==
\subsection{Discussions}\label{sec:sec_discussions}
\stitle{Impact of \decoprompt on correct-premise questions}
\begin{table*}[t!]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method    & \% true & \% false & \% true (GPT-judge) & BLEURT & ROUGE & BLEU \\\midrule
Original   &                                                                 &          &                     &        &       &      \\
Paraphrase &                                                                 &          &                     &        &       &      \\
\decoprompt &                                                                 &          &                     &        &       &     \\\bottomrule
\end{tabular}%
% }
\caption{Performance on generation task of TruthfulQA when \emph{Llama2-7b-chat} is prompted with original, paraphrased and decoprompt (paraphrase with lowest entropy) questions. }
\label{tab:correct_premise}
\end{table*}

Prior literature finds that hallucination mitigation strategies, such as adding an explicit false premise check in the prompt, could hurt performance on questions with valid premises~\citep{vu2023freshllms}. We study the impact of selecting the low-entropy paraphrase as the new prompt proposed by \decoprompt on the main generation task of TrutufulQA~\citep{lin2021truthfulqa}, which consists of a test set of $817$ factually correct questions written by humans. 


\stitle{Effectiveness of \decoprompt on existing false-premise dataset}
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
Method     & Llama2-7b-chat & Vicuna-7b & Qwen-7b-chat \\\midrule
Original   &                &           &              \\
\demoprompt &                &           &        \\\bottomrule     
\end{tabular}%
}
\caption{Accuracy of demoprompt on existing false-premise examples from FreshQA.}
\label{tab:freshqa_performance}
\end{table}
Existing false-premise datasets neglect to measure whether the tested LLM possesses the required factual knowledge or not, making it hard to diagnose the hallucination outcomes due to multiple counterfactors~\citep{varshney2023stitch,vu2023freshllms}. Encouraged by the reduced hallucination by \decoprompt, we further evaluate its effectiveness on false premises from FreshQA, which contains 136 questions that LLMs of different scales struggle on~\citep{vu2023freshllms}. We follow the relaxed human evaluation procedure to measure whether the main answer is correct.


